Coded Transaction Broadcasting for High-throughput Blockchains

High-throughput blockchains require efficient transaction broadcast mechanisms that can deliver transactions to most network nodes with low bandwidth overhead and latency. Existing schemes coordinate transmissions across peers to avoid sending redundant data, but they either incur a high latency or are not robust against adversarial network nodes. We present Strokkur, a new transaction broadcasting mechanism that provides both low bandwidth overhead and low latency. The core idea behind Strokkur is to avoid explicit coordination through randomized transaction coding. Rather than forward individual transactions. Strokkur nodes send out codewords -- XOR sums of multiple transactions selected at random. Since almost every codeword is useful for the receiver to decode new transactions, Strokkur nodes do not require coordination, for example, to determine which transactions the receiver is missing. Strokkur's coding strategy builds on LT codes, a popular class of rateless erasure codes, and extends them to support multiple uncoordinated senders with partially-overlapping continual streams of transaction data. Strokkur introduces mechanisms to cope with adversarial senders that may send corrupt codewords, and a simple rate control algorithm that enables each node to independently determine an appropriate sending rate of codewords for each peer. Our implementation of Strokkur in Golang supports 647k transactions per second using only one CPU core. Our evaluation across a 19-node Internet deployment and large-scale simulation show that Strokkur consumes 2--7.6x less bandwidth than the existing scheme in Bitcoin, and 9x lower latency that Shrec when only 4% of nodes are adversarial.

==> background.tex <==
\subsection{Distributed source coding}

Before diving deeper, it is useful to connect transaction broadcasting to the distributed source coding problem. It will make clear why coding is an ideal solution to transaction broadcasting, and justify our key design choices, including the decision to use LT codes.



Distributed source coding (DSC) considers this problem constrained on that the sources cannot communicate with each other. Indeed, this is the case in a blockchain. The topology of the peer-to-peer network is sparse, so a direct link between any pair in $P_1, P_2, \dots, P_d$ is unlikely. Routing through indirect links is also impractical: the network is unstructured to avoid targeted attacks~\cite{ethereum-eclipse}, so there is no routing table to compute an efficient route between two nodes.

One extreme of this problem is trivial: if $P_1, P_2, \dots, P_d$ had disjoint sets of transactions, then each source should send all of its transactions to $R$ as-is. Transaction broadcasting sits at the other extreme of this problem. Because $P_1, P_2, \dots, P_d$ are themselves blockchain nodes, they will eventually receive every transaction in the system. That is, any transaction that appears in source $P_i$ will eventually appear in all of $P_1, P_2, \dots, P_d$.




\ly{the controller solves two problems: (1) bootstrapping (chicken and egg), (2) adapting to changing load}

An alternative view of this problem is \textit{scheduling}. \ly{bitcoin/shrec: inefficient scheduling, erlay: efficient scheduling, DSC: no need for scheduling. DSC is the correct way to view this problem.}

an extension is network coding. but it does not work

\ly{don't say that the coding window of all sources are overlapping at any moment. we use a window of 50. at 2500 tps, it refreshes every 0.02 s. instead, say that a codeword received by one source is quickly received by all sources}

\ly{make clear that network coding does not work! and it is LT, and that we do not break down transactions, makes DSC work. otherwise the problem is better viewed as NC.}

\subsection{Choosing a code}

\label{sec:background-choose-code}

The purpose of using coding in \name is to eliminate the need for coordination between nodes. This presents a key requirement for the code we use.  

\name imposes \ly{come back for a number} key requirements on the choice of a code. First, codewords generated by multiple peers must be compatible with each other. A \name node connects to many peers, and receives codewords from all of them simultaneously. (It is unsafe for a node to only receive from one peer. If so, that peer would have total control over what the node can see, opening up possibilities for censorship.) The codewords, then  If   must be able to combine codewords from multiple peers.

Second, nodes must be able to generate codewords without communicating with each other.

the decoder must not be affected by a malicious peer.  

\subsection{LT codes primer}
\label{sec:background-lt}

\subsection{Adapting LT codes for \name Challenges in applying LT codes}
\label{sec:background-challenges}




We need to (1) combining multiple senders (2) some senders may be malicious. Say what is the property that we need: chance to examine a transaction before using it.

This makes almost all codes unapplicable. For example: RS does not work.

\noindent\textbf{LT codes.} We build on LT because it has the property. Explain quickly what is LT code and why it works. Make it short.

Mention the distribution, cite the paper.

\noindent\textbf{Challenges in using LT codes in \name.}

list challenges: it is nontrivial to just copy paste LT code. for example, windowing is not used before. All previous usages assumes a finite buffer of bytes. We have an infinite stream, so it is a new problem for us. also, we treat each transaction as a symbol

rate control

identifiers cost: it only appears in our app because we do not use LT to transmit a normal file

minimize coding delay

challenge: the transaction is not big enough to be broken up and coded. as a solution, we code multiple transactions together.

==> discussions.tex <==
\section{Discussion}
\label{sec:discussion}



==> node-anatomy.tex <==
\tikzstyle{encoder} = [draw, fill=blue!20, rectangle, 
    minimum height=2em, minimum width=4em, text centered, text width=4em]
\tikzstyle{decoder} = [draw, fill=red!20, rectangle, minimum height=2em, minimum width=4em, text centered, text width=4em]

\begin{tikzpicture}[auto, node distance=4cm, >=latex']
    \node [encoder] (enc1) {Encoder};
    \node [decoder, below of=enc1] (dec1) {Decoder};
    \node [encoder, left of=enc1] (enc2) {Encoder};
    \node [decoder, below of=enc2] (dec2) {Decoder};
    \draw [->] (dec1) -- (dec2);
    \draw [->] (dec2) -- (dec1);
  


\end{tikzpicture}
